A spatially resolved radio spectral study of the galaxy M 51

Radio continuum emission from galaxies at gigahertz frequencies can be used as an extinction-free tracer of star formation. However, at frequencies of a few hundred megahertz, there is evidence for low-frequency spectral flattening. We wish to better understand the origin of this low-frequency flattening and, to this end, perform a spatially resolved study of the nearby spiral galaxy M 51. We explore the different effects that can cause flattening of the spectrum towards lower frequencies, such as free-free absorption and cosmic-ray ionisation losses. We used radio continuum intensity maps between 54 and 8350 MHz at eight different frequencies, with observations at 240 MHz from the Giant Metrewave Radio Telescope presented for the first time. We corrected for contribution from thermal free-free emission using an H$\alpha$ map that has been extinction-corrected with 24 $\mu$m data. We fitted free-free absorption models to the radio spectra to determine the emission measure (EM) as well as polynomial functions to measure the non-thermal spectral curvature. The non-thermal low-frequency radio continuum spectrum between 54 and 144 MHz is very flat and even partially inverted, particularly in the spiral arms; contrary, the spectrum at higher frequencies shows the typical non-thermal radio continuum spectrum. However, we do not find any correlation between the EMs calculated from radio and from H$\alpha$ observations; instead, the non-thermal spectral curvature weakly correlates with the HI gas mass surface density. This suggests that cosmic-ray ionisation losses play an important role in the low-frequency spectral flattening. The observed spectral flattening towards low frequencies in M 51 is caused by a combination of ionisation losses and free-free absorption. The reasons for this flattening need to be understood in order to use sub-GHz frequencies as a star-formation tracer.

==> BIBdef.tex <==
\newcommand{\aj}{AJ}% 
          % Astronomical Journal 
\newcommand{\araa}{ARA\&A}% 
          % Annual Review of Astron and Astrophys 
\newcommand{\apj}{ApJ}% 
          % Astrophysical Journal 
\newcommand{\apjl}{ApJ}% 
          % Astrophysical Journal, Letters 
\newcommand{\apjs}{ApJS}% 
          % Astrophysical Journal, Supplement 
\newcommand{\ao}{Appl.~Opt.}% 
          % Applied Optics 
\newcommand{\apss}{Ap\&SS}% 
          % Astrophysics and Space Science 
\newcommand{\aap}{A\&A}% 
          % Astronomy and Astrophysics 
\newcommand{\aapr}{A\&A~Rev.}% 
          % Astronomy and Astrophysics Reviews 
\newcommand{\aaps}{A\&AS}% 
          % Astronomy and Astrophysics, Supplement 
\newcommand{\azh}{AZh}% 
          % Astronomicheskii Zhurnal 
\newcommand{\baas}{BAAS}% 
          % Bulletin of the AAS 
\newcommand{\jrasc}{JRASC}% 
          % Journal of the RAS of Canada 
\newcommand{\memras}{MmRAS}% 
          % Memoirs of the RAS 
\newcommand{\mnras}{MNRAS}% 
          % Monthly Notices of the RAS 
\newcommand{\pra}{Phys.~Rev.~A}% 
          % Physical Review A: General Physics 
\newcommand{\prb}{Phys.~Rev.~B}% 
          % Physical Review B: Solid State 
\newcommand{\prc}{Phys.~Rev.~C}% 
          % Physical Review C 
\newcommand{\prd}{Phys.~Rev.~D}% 
          % Physical Review D 
\newcommand{\pre}{Phys.~Rev.~E}% 
          % Physical Review E 
\newcommand{\prl}{Phys.~Rev.~Lett.}% 
          % Physical Review Letters 
\newcommand{\pasp}{PASP}% 
          % Publications of the ASP 
\newcommand{\pasj}{PASJ}% 
          % Publications of the ASJ 
\newcommand{\qjras}{QJRAS}% 
          % Quarterly Journal of the RAS 
\newcommand{\skytel}{S\&T}% 
          % Sky and Telescope 
\newcommand{\solphys}{Sol.~Phys.}% 
          % Solar Physics 
\newcommand{\sovast}{Soviet~Ast.}% 
          % Soviet Astronomy 
\newcommand{\ssr}{Space~Sci.~Rev.}% 
          % Space Science Reviews 
\newcommand{\zap}{ZAp}% 
          % Zeitschrift fuer Astrophysik 
\newcommand{\nat}{Nature}% 
          % Nature 
\newcommand{\iaucirc}{IAU~Circ.}% 
          % IAU Cirulars 
\newcommand{\aplett}{Astrophys.~Lett.}% 
          % Astrophysics Letters 
\newcommand{\apspr}{Astrophys.~Space~Phys.~Res.}% 
          % Astrophysics Space Physics Research 
\newcommand{\bain}{Bull.~Astron.~Inst.~Netherlands}% 
          % Bulletin Astronomical Institute of the Netherlands 
\newcommand{\fcp}{Fund.~Cosmic~Phys.}% 
          % Fundamental Cosmic Physics 
\newcommand{\gca}{Geochim.~Cosmochim.~Acta}% 
          % Geochimica Cosmochimica Acta 
\newcommand{\grl}{Geophys.~Res.~Lett.}% 
          % Geophysics Research Letters 
\newcommand{\jcp}{J.~Chem.~Phys.}% 
          % Journal of Chemical Physics 
\newcommand{\jgr}{J.~Geophys.~Res.}% 
          % Journal of Geophysics Research 
\newcommand{\jqsrt}{J.~Quant.~Spec.~Radiat.~Transf.}% 
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer 
\newcommand{\memsai}{Mem.~Soc.~Astron.~Italiana}% 
          % Mem. Societa Astronomica Italiana 
\newcommand{\nphysa}{Nucl.~Phys.~A}% 
          % Nuclear Physics A 
\newcommand{\physrep}{Phys.~Rep.}% 
          % Physics Reports 
\newcommand{\physscr}{Phys.~Scr}% 
          % Physica Scripta 
\newcommand{\planss}{Planet.~Space~Sci.}% 
          % Planetary Space Science 
\newcommand{\procspie}{Proc.~SPIE}% 
          % Proceedings of the SPIE 
\endinput
